Reward Learning from Narrated Demonstrations

Humans effortlessly "program" one another by communicating goals and desires in natural language. In contrast, humans program robotic behaviours by indicating desired object locations and poses to be achieved, by providing RGB images of goal configurations, or supplying a demonstration to be imitated. None of these methods generalize across environment variations, and they convey the goal in awkward technical terms. This work proposes joint learning of natural language grounding and instructable behavioural policies reinforced by perceptual detectors of natural language expressions, grounded to the sensory inputs of the robotic agent. Our supervision is narrated visual demonstrations(NVD), which are visual demonstrations paired with verbal narration (as opposed to being silent). We introduce a dataset of NVD where teachers perform activities while describing them in detail. We map the teachers' descriptions to perceptual reward detectors, and use them to train corresponding behavioural policies in simulation.We empirically show that our instructable agents (i) learn visual reward detectors using a small number of examples by exploiting hard negative mined configurations from demonstration dynamics, (ii) develop pick-and place policies using learned visual reward detectors, (iii) benefit from object-factorized state representations that mimic the syntactic structure of natural language goal expressions, and (iv) can execute behaviours that involve novel objects in novel locations at test time, instructed by natural language.

==> lgold.tex <==
\subsection{Language grounding for reward learning}



%NL utterances in our video narrations usually have two main intentions: (i) to describe/refer to objects and actions in the scene, and, (ii) to contribute information regarding temporal and causal  relationships in the actions. 
We focus on grounding NL descriptions regarding spatial object arrangements, \eg, \textit{``the apple is to the left of the white plate''}. Corresponding reward detectors will be used to train pick-and-place policies for novel goals instructable by NL, e.g.,  \textit{``the orange should be inside the bowl''}. % , providing agents instructable by NL to move objects around. 

%to part of our dataset that aims to teach regarding spatial relationship between objects,

%Our goal is to learn visual detectors that can localize the subject and objects of referring expressions, which we assume describe a large set of desired post-conditions of pick and place behaviours. 

What is the right neural architecture for detecting NL utterances describing object arrangements? Recent work of \citep{modularreferential} proposed a modular neural architecture that scores bounding boxes and their arrangements, based on how well they match an input NL referential expression.
%We build upon previous work of .... \etal \cite{} that localizes referring expressions in static images by considering the graph comprised of the object and subject nodes, and the edge features as ncoding their spatial arrangement. 
%structure, and adding three scores, two unary scores for the object and subject, and one score for the relative spatial arrangement of the two bounding boxes. 
%Specifically, the referring expression detector is a modular neural architecture, that given a referring expression and an object and subject bounding box hypotheses predicts a score that the hypotheses and their arrangement match the referring expression.
Their model combines two localization (i.e., object detector) modules (for both the subject and the object), and one relation module for their spatial relation, as shown in Figure \ref{fig:referential}. Input to each  module is a vector embedding of the subject, object and relation respectively, computed using a Bidirectional LSTM network over the word embeddings of the referential phrases. The vector embedding of each of the three entities is computed using a weighted average over the hidden states vectors of the individual words, where three weight distributions are predicted by the BiLSTM separately for the object, the subject, and the relation. 
Along with the linguistic entity vector, the localization module takes as input (deep) visual features extracted from the box hypothesis, while the relation module operates on the spatial features of the two bounding boxes, encoded as normalized pixel coordinates. In that work, the model is trained end-to-end (without supervising the language model with subject, object, or relation annotations) to localize referential expressions in the Visual Genome dataset \cite{krishnavisualgenome}. 
Although a referential expression, e.g., ``the orange in the bowl", is not identical in meaning to a description, e.g., ``the orange is in the bowl", or to a desired post-condition, e.g., ``the orange should be in the bowl", in practice their learned embeddings are similar. 

%We first observed that training the referring expression network on Visual genome was not sufficient to provide correct scores for the examples in our dataset. Our explanation for this is the following \todo{Fish}.


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/fig2.pdf}
     \centering
        \caption{Modular network of \cite{modularreferential} for detecting referential expressions, used in our work. Inputs are depicted in blue boxes, and outputs are in red; gray boxes are neural network layers and operations.
    }
    \label{fig:referential}
\end{figure}





\paragraph{Unpaired supervision}
The model of Hu \etal \cite{modularreferential} is trained in the Visual Genome dataset \cite{krishnavisualgenome}, using neural weights of the localization modules pretrained on ImageNet \cite{imagenet_cvpr09}. We achieve better localization accuracy by further training our localization modules in the object detection dataset of COCO \cite{DBLP:journals/corr/LinMBHPRDZ14}. 
COCO has annotated bounding boxes in static images with corresponding object category labels, not referential expressions. 
%To be able to exploit rich supervised annotation of object detectors in COCO, 
For each object in COCO, we sample dummy (but plausible) referential expressions and descriptions. We train the localization module using data from both Visual Genome and COCO.
%We sample for each annotated bounding box example a dummy yet plausible referential expression or description, and trained the localization module  using both data from Visual Genome and COCO.
%, so that the COCO object category vocabulary and numerous annotated images will be used to improve accuracy of the localization modules. 


\paragraph{Weakly supervised training using multiple instance learning}
We finetune both the localization and the relation module of our reward detector in our narrated videos using multiple instance learning. 
Each video frame in Teach-a-Toddler is annotated with the corresponding piece of the  automatically obtained transcript %using the publicly available Google Speech API \cite{googlespeech}. The transcript is  segmented into four to five second chunks. Sparse mistakes made by the speech recognizer are corrected manually by the demonstrators. 
%Each video frame is annotated by the corresponding transcript piece assigned automatically by the speech recognizer. 
Our modular visual-linguistic detector \cite{modularreferential}  operates directly on this automatically obtained  utterance-frame alignment. We consider only the frames paired with exactly one NL utterance. 


%Let \scsubject, \scobject and \screlation \ denote the scores of our reward detector for the subject, object and relation of a NL utterance describing spatial object configurations. 

  We then request each of the individual localization and relation modules, as well as the full detector, to score higher in the frames where the annotation is available and lower on frames where such annotation is not present:
 
In each video frame, our region proposal network \cite{DBLP:journals/corr/LiuAESR15} predicts a set of bounding box proposals. 
%We consider the following 
Let $k$ denote the frame index, $\BB_k$ the set of bounding box proposals in frame $k$, $\nl_k$ denote the NL utterance in frame $k$ that describes an object spatial configuration, $\vsubj_k$, $\vobj_k$, $\vrel_k$ the hidden state vectors from BiLSTM for the subject, object, and relation, $b_i$ the spatial features of the $i$th bounding box proposal, and $f_i$ the deep visual features pooled from the $i$th bounding box proposal. Then, the score of our  detector in frame $k$ reads:
\begin{equation}
    \mathcal{S}_k^{\nl_k} = \max_{i,j, i \neq j} loc(\vsubj_k, f_i)+loc(\vobj_k, f_j)+rel(\vrel_k, b_i,b_j). \nonumber
\end{equation}

Our training loss asks for the score of our model for a particular utterance to be higher for the paired frame, and lower for any other frame $\ell$ paired with different NL utterance. Our loss function reads:
\begin{equation}
    \mathcal{L} = \sum_\ell \sum_k \max(0, \mathcal{S}_\ell^{\nl_k} -\mathcal{S}_k^{\nl_k}).  
\end{equation}

In frames where our localization module scores have low entropy,  indicating the presence of a known object category, we use detected subject and object boxes to determine the score of the relation module:


\begin{align}
    \mathcal{S}_k^{rel_k} =& rel(\vrel_k, b_i,b_j), \\
    i=&\argmax_{i=1 \cdots |\BB_k|} loc(\vsubj_k, f_i), \nonumber \\ j=&\displaystyle \argmax_{j=1 \cdots |\BB_k|} loc(\vobj_k, f_j). 
\end{align}

We then  train the relation module alone using a similar metric learning loss:

\begin{equation}
    \mathcal{L}^{rel} = \sum_\ell \sum_k \max(0, \mathcal{S}_\ell^{rel_k} -\mathcal{S}_k^{rel_k}),  
\end{equation}
where

\begin{align}
    \mathcal{S}_\ell^{rel_k} =& rel(\vrel_k, b_i,b_j), \\
    i=&\argmax_{i=1 \cdots |\BB_\ell|} loc(\vsubj_\ell, f_i), \nonumber \\ j=&\displaystyle \argmax_{j=1 \cdots |\BB_\ell|} loc(\vobj_\ell, f_j). 
\end{align}


%by decomposing the score of the three modules, as opposed to adding them up, to avoid overfitting. The reasoning is that when the correct spatial configuration is achieved the relation module cannot ``cheat" by using scores of the localization module. 

 We  train our relation module with data augmentation, by slightly jittering the locations and sizes of the objects in the scene during training. We did not consider data augmentation for the localization modules. Our finetuned model benefits from the fact that the  demonstrator uses the same pair of objects to diverse configurations, providing hard negatives for the relation module. In contrast, static image datasets collected from the Internet cannot benefit from such controlled configuration generation to fight biases.%Multiple instance consider data augmebtation by jittering our o

%while in Visual Genome suffers from world bias: the rider is usually on top of the bike, as opposed to its right. %and thus we can find examples where the 

%\todo{we need an MIL equation here without bugs...}


%The above training procedure results correct score fluctuations of the relation module.

%We did not need to finetune the linguistic parser, though that would have been possible, since the simple and canonical language used in our narrated videos, allows of-the-shelf parser, such as, SyntaxNet \cite{}, to achieve very high accuracy localizing object and sibject of spatial modifiers. Note that this is the advantage of our dataset, purposfully collected for teaching/instructing a neural model, as opposed to teaching cooking to adults. Intrestingly, such simplicity of our natural utterances can easily be augmented using paraphrasing and map our video scene with way more ambiguity, complex, and elliptic description \cite{}, for learnign to handle complexity of NL. This is though beyond the scope of the current work.




